Gradient Reweighting: Towards Imbalanced Class-Incremental Learning

Class-Incremental Learning (CIL) trains a model to continually recognize new classes from non-stationary data while retaining learned knowledge. A major challenge of CIL arises when applying to real-world data characterized by non-uniform distribution, which introduces a dual imbalance problem involving (i) disparities between stored exemplars of old tasks and new class data (inter-phase imbalance), and (ii) severe class imbalances within each individual task (intra-phase imbalance). We show that this dual imbalance issue causes skewed gradient updates with biased weights in FC layers, thus inducing over/under-fitting and catastrophic forgetting in CIL. Our method addresses it by reweighting the gradients towards balanced optimization and unbiased classifier learning. Additionally, we observe imbalanced forgetting where paradoxically the instance-rich classes suffer higher performance degradation during CIL due to a larger amount of training data becoming unavailable in subsequent learning phases. To tackle this, we further introduce a distribution-aware knowledge distillation loss to mitigate forgetting by aligning output logits proportionally with the distribution of lost training data. We validate our method on CIFAR-100, ImageNetSubset, and Food101 across various evaluation protocols and demonstrate consistent improvements compared to existing works, showing great potential to apply CIL in real-world scenarios with enhanced robustness and effectiveness.

==> sec/method_old.tex <==

\section{Method}
\label{sec:method}
In this section, we illustrate our proposed gradient reweighting to address both intra-phase class-imbalance in Section~\ref{subsec: intra-phase} and then extend it for inter-phase class-imbalance in Section~\ref{subsec: inter-phase}.


\subsection{Intra-Phase Class-Imbalance}
\label{subsec: intra-phase}
As illustrated in Section~\ref{sec:prelim}, the severe class-imbalanced data distribution among each new task $\mathcal{T}^t$ poses significant challenges for learning new knowledge due to skewed optimization process caused by imbalanced gradients between instance-rich and instance-rare classes. The objective is to mitigate the intra-phase imbalance issue by re-weighting the gradient to enable the learning of an unbiased classifier. Specifically, consider the case of learning the first task $\mathcal{T}^1 = \{\mathcal{X}^1, \mathcal{Y}^1\}$ from a scratch model $\mathcal{M}^0(f_\theta, W)$ where $f_\theta$ and $W$ refers to the feature extractor and classifier, respectively. The cross-entropy loss is formulated as 
\begin{equation}
\label{eq: cn}
    \begin{aligned}
        \mathcal{L}_{ce} = - \frac{1}{|\mathcal{X}^1|}\sum_{k=1}^{|\mathcal{X}^1|} \sum_{j=1}^{|\mathcal{Y}^1|}\hat{y}_j \log(p_j)
    \end{aligned}
\end{equation}
where $p_j$ is the Softmax of the $j$th output logit $z_j = [W^Tf_\theta(\textbf{x}_k])]_j$ and $\hat{y}_j$ is the one-hot label. Motivated by the imbalanced gradients as indicated in Equation~\ref{eq: gradeint_update}, we introduce a class-balance ratio $\alpha$ for each class $j \in \mathcal{Y}^1$ as
\begin{equation}
\label{eq: intra-phase}
    \begin{aligned}
        W_{i+1}^{j} = W_i^{j} - \eta \alpha^{j}_i \nabla_{\mathcal{L}_{ce}}(W_i^{j}) 
    \end{aligned}
\end{equation}
However, it could be non-trivial to obtain the appropriate class-balance ratio due to the intricate data-dependent optimization process. In this work, we propose a simple yet effective solution to calculate the ratio by leveraging historical gradient magnitudes. In detail, 
we calculate the ratio $\alpha_i$ at iteration $i$ based on the accumulated magnitude of gradients corresponding to each class $j$ as 
\begin{equation}
\label{eq: alpha-intra-phase}
    \begin{aligned}
    \alpha^{j}_i = \frac{\underset{m \in \mathcal{Y}^1}{\textit{min}}\Phi^m_i}{\Phi^{j}_i}, \quad 
        \Phi^{j}_i = \sum_{k=1}^i ||\nabla_{\mathcal{L}_{ce}}(W_k^{j})||
    \end{aligned}
\end{equation}
By doing so, we dynamically recalibrate the weight updates, ensuring that both majority and minority classes contribute equally to the learning process and address the biased issue. 

\subsubsection{Regularized Softmax Output}
\label{subsubsec: regularization}
The main goal of gradient re-weighting is to reduce the effect of imbalanced optimization between head and tail classes by down-weighting the weight updates of head classes. However, while this adjustment helps in emphasizing tail classes, it also inadvertently leads to increased loss values for the head classes, resulting in larger gradients. Specifically, the gradient of a head class input image $(\textbf{x}_k, y_k)$ with respect to each class $j \in \mathcal{Y}^1$ can be calculated as 
\begin{equation}
\label{eq: gradients}
    \frac{\partial \mathcal{L}_{ce}}{\partial z_j} = 
    \left\{ \begin{array}{ccl}
    p_{j} -1 & j = y_k \\ p_{j} & j \neq y_k
    \end{array}\right., p_j = \frac{exp(z_j)}{\sum_{m = 1}^{|\mathcal{Y}^1|}exp(z_m)}
\end{equation}
where $z_j$ is the $j$th output logit and $p_j$ is the corresponding softmax output. Attributing to the down-weight of head class gradients, the output value of $z_{y_k}$ decreases during the training process. Consequently, it results in an increase of the positive gradient norm $||1 - p_j||$, prompting the head class weight $W^{y_k}$ to produce a higher output logit value. Concurrently, since the total sum of softmax outputs is constrained to 1, the decrease of $z_{y_k}$ leads to the rise of the negative gradient norm $||p_j||$, driving the tail classes weight to output even lower scores. Motivated by~\cite{logit_adjust}, we alleviate this issue by adjusting the softmax cross-entropy output logits as in Equation~\ref{eq:r-softmax}
\begin{equation}
\label{eq:r-softmax}
    \begin{aligned}
    p_j = \frac{exp(z_j + \log \pi_j)}{\sum_{m = 1}^{|\mathcal{Y}^1|}exp(z_m + \log \pi_m)}
    \end{aligned}
\end{equation}
where $\log \pi_j$ is the per-label offsets added to the original output logit. Generally, the instance-rich classes have larger $\pi_j$ with an increase of softmax output $p_j$ to compensate for the side effect of down-weighting the gradients during the training process. In this work, we propose to use the accumulated gradient norm in Equation~\ref{eq: gradients} to calculate $\pi_j$ at each iteration $i$ as 
\begin{equation}
\label{eq:offset}
    \begin{aligned}
    \pi_j = \frac{\Phi^{j}_i}{\sum_{m = 1}^{|\mathcal{Y}^1|} \Phi^{m}_i}
    \end{aligned}
\end{equation}



% algorithm block -----------------

% \begin{algorithm}[t]
% \caption{Gradient Reweighting}\label{alg:gr}
% \begin{small} 
%     \hspace*{0.02in} {\bf Input:}
%     A new tasks: $\mathcal{T}^t$\\
%     \hspace*{0.02in} {\bf Require:} 
%     CIL model $\mathcal{M}^{t-1}(f_\theta, W)$, learning rate $\eta$\\
% \vspace{-0.35cm}
% \begin{algorithmic}[1]
% \State Initialize $\Phi^{j}, j\in \mathcal{Y}^{1:t}$  \Comment{accumulated gradients}
% \For{i = 1, 2, ... } \Comment{iteration index}
% \State $\Phi^{j}_i \leftarrow \Phi^{j}_i +  ||\nabla_{\mathcal{L}_{ce}}(W_i^{j})||$
% \If {$t = 1$}  \Comment{intra-phase imbalance}
% \State $\alpha_i^j \leftarrow \underset{m \in \mathcal{Y}^t}{\textit{min}}\Phi^m_i/\Phi^{j}_i  $ \Comment{balance ratio}
% \State $W_{i+1}^{j} \leftarrow W_i^{j} - \eta \alpha^{j}_i \nabla_{\mathcal{L}_{ce}}(W_i^{j}) $ \Comment{\textit{back prop}}
% \Else \Comment{inter and intra-phase imbalance}
% % \State $r_i \leftarrow |\mathcal{Y}^{t}|\sum_{j \in \mathcal{Y}^{1:t-1}}\Phi_i^j/|\mathcal{Y}^{1:t-1}|\sum_{j \in \mathcal{Y}^{t}}\Phi_i^j$ \Comment{task balance ratio}
% \State $r_i \leftarrow \frac{\frac{1}{|\mathcal{Y}^{1:t-1}|} \sum_{j \in \mathcal{Y}^{1:t-1}}\Phi_i^j}{\frac{1}{|\mathcal{Y}^{t}|} \sum_{j \in \mathcal{Y}^{t}}\Phi_i^j}$ \Comment{task balance ratio}
% \State $\alpha_i^j \leftarrow r_i \times \underset{m \in \mathcal{Y}^{1:t-1}}{\textit{min}}\Phi^m_i/\Phi^{j}_i$
% \Comment{old classes}
% \State $\alpha_i^j \leftarrow \underset{m \in \mathcal{Y}^{t}}{\textit{min}}\Phi^m_i/\Phi^{j}_i$
% \Comment{new classes}
% \State $\beta_i \leftarrow \frac{\sum_{j\in \mathcal{Y}^{1:t}} \alpha_i^j \nabla_{\mathcal{L}_{ce}}}{\sum_{j\in \mathcal{Y}^{1:t-1}} \nabla_{\mathcal{L}_{DAKD}}}$ \Comment{loss balance ratio}
% \State $W_{i+1}^{j} \leftarrow W_i^{j} - \eta (\alpha^{j}_i \nabla_{\mathcal{L}_{ce}}(W_i^{j}) + \beta_{i} \nabla_{\mathcal{L}_{kd}}(W_i^{j}))$
% \EndIf
% \EndFor
% \State $\mathcal{M}^{t} \leftarrow \mathcal{M}^{t-1}$ \Comment{$\mathcal{T}^t$ finished}
% \end{algorithmic}
% \label{alg:online sampler}
% \end{small}
% \end{algorithm} 
% algorithm block -----------------


\subsection{Inter-Phase Class-Imbalance}
\label{subsec: inter-phase}
Now, consider the case when learning a new task $\mathcal{T}^t(t>1)$ with the present of learned classes belonging to $\mathcal{Y}^{1:t-1}$. The challenges in this case arise from two main perspectives. First, the training distribution, denoted as $\mathcal{D}$, varies for already learned classes where $\mathcal{D}(\mathcal{X}_e^{1:t-1}, \mathcal{Y}_e^{1:t-1}) \neq \mathcal{D}(\mathcal{X}^{1:t-1}, \mathcal{Y}^{1:t-1})$ as only limited exemplars are stored for training in subsequent learning phases after they were initially observed. Therefore, simply balancing all gradients without accounting for this will result in knowledge loss for learned classes. Second, the training objectives vary between new and old tasks where the learned tasks $\mathcal{T}^{1:t-1}$ build upon knowledge accumulated from previous learning phases, while the new task $\mathcal{T}^{t}$ starts from scratch without any prior knowledge. Consequently, balancing the gradient updates may not be effective due to the intrinsic imbalance optimization objectives, which require a more adaptive and flexible approach to ensure the model can effectively learn new tasks without forgetting the knowledge from previous ones. 

To this end, we extend our method illustrated in Section~\ref{subsec: intra-phase} to address the inter-phase imbalance by adding two components including (i) a Distribution-Aware Knowledge Distillation (DAKD) loss to maintain the information from original training distribution while mitigating the imbalanced forgetting issue, and (ii) a Decoupled Gradient Reweighting (DGR) framework to separately manage the gradients between new and already learned tasks to ensure a balance between the stability of past knowledge and the plasticity required for learning new classes,  which will be illustrated in Section~\ref{subsubsec: im-forgetting} and~\ref{subsubsec: integrated gradient}, respectively. 



% separately re-weighting the gradients for previously learned tasks $\mathcal{T}^{1:t-1}$ and the new task $\mathcal{T}^{t}$ where we integrate the prior information using task accumulated gradients. Additionally, we include the knowledge distillation loss~\cite{KD} to strike a balance with the cross-entropy loss from the objective of ensuring stability (to preserve previously acquired knowledge) and allowing plasticity (to effectively adapt to new classes). 

% Specifically, we calculate the balance ratio $\alpha$ as in Equation~\ref{eq: aplha-inter}. 
% \begin{equation}
% \label{eq: aplha-inter}
%     \alpha^j_i = 
%     \left\{ \begin{array}{rcl}
%     \frac{\underset{m \in \mathcal{Y}^{1:t-1}}{\textit{min}}\Phi^m_i}{\Phi^{j}_i} & j \in \mathcal{Y}^{1:t-1} \\  r_i \times \frac{\underset{m \in \mathcal{Y}^t}{\textit{min}}\Phi^m_i}{\Phi^{j}_i} & j \in \mathcal{Y}^{t}
%     \end{array}\right.
% \end{equation}
% The $\Phi^j_i$ is the iteration accumulated gradients as in Equation~\ref{eq: alpha-intra-phase} and $r_i$ is the ratio at iteration $i$ to balance the new and learned classes using the mean of accumulated gradients as
% \begin{equation}
% \label{eq:ri}
%     \begin{aligned}
%     r_i = \frac{\frac{1}{|\mathcal{Y}^{t}|} \sum_{j \in \mathcal{Y}^{t}}\Phi_i^j}{\frac{1}{|\mathcal{Y}^{1:t-1}|} \sum_{j \in \mathcal{Y}^{1:t-1}}\Phi_i^j}
%     \end{aligned}
% \end{equation}
% Later in Section~\ref{subsec: ablation}, we will show that directly calculate $\alpha_j$ using Equation~\ref{eq: alpha-intra-phase} on all classes without separating them can lead to under-fitting of the new classes. 

\subsubsection{Distribution-Aware Knowledge Distillation}
\label{subsubsec: im-forgetting}
Similar to~\cite{BiC, mainatining}, we consider adding the knowledge distillation loss~\cite{KD} to maintain the learned knowledge due to the changing of training distribution for learned classes. The original distillation loss can be expressed as 
\begin{equation}
\label{eq: kd}
    \begin{aligned}
        \mathcal{L}_{kd} = - \frac{1}{|\mathcal{X}^{t}+\mathcal{X}_e^{1:t-1}|}\sum_{k=1}^{|\mathcal{X}^{t}+\mathcal{X}_e^{1:t-1}|} \sum_{j=1}^{|\mathcal{Y}^{1:t-1}|}\hat{p}_j \log(p_j)
    \end{aligned}
\end{equation}
where $\hat{p}_j$ denotes the Softmax output of $\hat{z}_j$ from the teacher model $\hat{M}^{t-1}$ with frozen parameters obtained in the last learning phase. 
However, as mentioned earlier in Section~\ref{sec:intro}, catastrophic forgetting can be imbalanced where a large volume of instances from the head class become unavailable in comparison to the tail class in the subsequent incremental learning phases due to the fixed memory budget. Though the most intuitive way to address this issue is storing more data for head classes and less data for tail classes, it poses another nontrivial challenge arising from a class-imbalanced exemplar set that potentially intensify both over-fitting and under-fitting issues. Therefore, we introduce the Distribution-Aware Knowledge Distillation (DAKD) to maintain the knowledge by taking into account the distribution of the lost training data. Specifically, we obtain the number of lost training data $s_j = |\mathcal{X}^j| - |\mathcal{X}_e^{j}|$ for each class $j \in \mathcal{Y}^{1:t-1}$ where $|\mathcal{X}^j|$ and $|\mathcal{X}_e^{j}|$ denote the number of original training data and stored exemplars for class $j$, respectively. Then we calculate the $\mathcal{L}_{DAKD}$ as 
\begin{equation}
\label{eq: decompkd}
    \begin{aligned}
        \mathcal{L}_{DAKD} = \sigma \mathcal{L}_{kd}^b (z,\hat{z})  + (1 - \sigma) \mathcal{L}_{kd}^{imb}(\tilde{z},\hat{z}) 
    \end{aligned}
\end{equation}
where we decompose the original $\mathcal{L}_{kd}$ into two parts using an imbalance factor $\sigma \in [0, 1]$ measured by the entropy of lost training data distribution. $\mathcal{L}_{kd}^b$ denotes the balanced part calculated using the original output logit $z$, and $\mathcal{L}_{kd}^{imb}$ denotes the imbalanced part with adjusted output logits $\tilde{z}$ determined by
\begin{equation}
\label{eq: z}
    \begin{aligned}
        \tilde{z}_j = \frac{s_j}{\sum_m^{|\mathcal{Y}^{1:t-1}|} s_m} z_j + (1 - \frac{s_j}{\sum_m^{|\mathcal{Y}^{1:t-1}|} s_m})\hat{z}_j 
    \end{aligned}
\end{equation}
where this calibrated distribution of output logits $\tilde{z}$ demonstrates larger discrepancy ($|\tilde{z}_j - \hat{z}_j|$) for classes $j$ with a higher volume of training data lost (\textit{i.e.}, head classes), thereby assigning those classes with more efforts for knowledge distillation compared to those with less data lost (\textit{i.e.}, tail classes) which only require a subtler distillation intervention to maintain the learned knowledge. This tailored logit adjustment ensures that the extent of knowledge distillation is appropriately aligned with the level of data lost experienced by each class. 
The overall loss function for learning a new task $\mathcal{T}^t, t>1$ can be expressed as 
\begin{equation}
\label{eq: z}
    \begin{aligned}
        \mathcal{L} = \mathcal{L}_{ce} + \lambda \mathcal{L}_{DAKD}
    \end{aligned}
\end{equation}
where $\lambda$ is the ratio to adjust the influence of knowledge distillation and we set $\lambda = \sqrt{|\mathcal{X}_{old}|/|\mathcal{X}_{new}|}$ in this work where $|\mathcal{X}_{old}|$ and $|\mathcal{X}_{new}|$ denote the total number of old and new classes training data seen so far. 

\begin{figure}[t]
\begin{center}
  \includegraphics[width=1.\linewidth]{fig/method.pdf}
  \caption{The illustration of Decomposed Gradient Reweighting (DGR) in imbalanced CIL, which balances the plasticity learning by separately adjusting gradients with class-balance ratios $\alpha$ and task-balance ratios $r$. Followed by tuning the stability-plasticity trade-off with a loss balance ratio $\beta$}
  \label{fig:method}
\end{center}
\end{figure}

\subsubsection{Decoupled Gradient Reweighting}
\label{subsubsec: integrated gradient}
The overview of Decoupled Gradient Reweighting (DGR) is shown in Figure~\ref{fig:method}, which addresses the inter-phase imbalance issue by striking a balance between stability (maintaining past knowledge) and plasticity (learning new classes). Generally, the gradients from cross-entropy loss ($\nabla_{\mathcal{L}_{ce}}$) in CIL represent the plasticity that enables the model to adapt to new training data distribution by incorporating both exemplars of old classes and the data from new classes. In contrast, the stability is introduced by the gradients from knowledge distillation loss ($\nabla_{\mathcal{L}_{DAKD}}$) to guide the model towards a solution that aligns with the training distribution from the previous learning phases. Therefore, the DGR address inter-phase imbalance in two folds by first reweighting the gradient $\nabla_{\mathcal{L}{ce}}$ from $\mathcal{L}_{ce}$ to ensure unbiased plasticity and then modulating the interaction between $\nabla{\mathcal{L}{ce}}$ and $\nabla{\mathcal{L}_{DAKD}}$ to attain a balanced equilibrium between plasticity and stability. 


\textbf{For plasticity}, instead of directly calculating the class-balance ratio $\alpha_j$ collectively on all classes as described in Section~\ref{subsec: intra-phase}, the DGR first separately considers the learned classes for $j \in \mathcal{Y}^{1:t-1}$ and new classes for $j \in \mathcal{Y}^{t}$ to calculate the class-balance ratios $\alpha_i^j$ respectively. Then, we multiply it with a task-balance ratio $r_i^j$ calculated by  
\begin{equation}
\label{eq:ri}
    \begin{aligned} r_i^j = 
\left\{ \begin{array}{ccl}
   \textit{min} \{1, \frac{1}{r_{\Phi_i}}\} & j \in \mathcal{Y}^{1:t-1} \\  \textit{min} \{1, r_{\Phi_i} \times exp( - \frac{|\mathcal{X}^{1:t-1}|}{|\mathcal{X}^{1:t}|}) \} & j \in \mathcal{Y}^{t}
    \end{array}\right.
    \end{aligned}
\end{equation}
where $exp( - \frac{|\mathcal{X}^{1:t-1}|}{|\mathcal{X}^{1:t}|})$ is the attenuation factor and $r_{\Phi_i}$ is the ratio of average accumulated gradients for learned classes to new classes as
\begin{equation}
\label{eq:ri}
    \begin{aligned}
    r_{\Phi_i} = \frac{ \frac{1}{|\mathcal{Y}^{1:t-1}|}\sum_{j \in \mathcal{Y}^{1:t-1}}\Phi_i^j}{ \frac{1}{|\mathcal{Y}^{t}|} \sum_{j \in \mathcal{Y}^{t}}\Phi_i^j}
    \end{aligned}
\end{equation}

The advantage of employing the attenuation factor lies in promoting a more equitable optimization based on the fact that the learned classes are built upon the knowledge learned in prior learning phases, whereas the new classes are being trained from scratch. Therefore, merely balancing the gradient contributions between new and old classes could inadvertently lead to the underfitting of new classes as they may not receive adequate training emphasis. Recognizing this, the attenuation factor adjusts the gradient reweighting ratio in favor of new classes proportional to the volume of data that has already been trained, thereby providing a calibrated boost in support of the new classes to mitigate the learning disparities. Later in Section~\ref{subsec: ablation}, we demonstrate that directly calculating $\alpha_j$ using Equation~\ref{eq: alpha-intra-phase} on all classes without DGR could potentially lead to under-fitting of the new classes. 


\textbf{For tuning between stability and plasticity}, we adjust the norm of gradients from distillation $||\nabla_{\mathcal{L}_{DAKD}}||$ to make it balance with cross-entropy $||\nabla_{\mathcal{L}_{ce}}||$ by including a loss balance ratio $\beta_i$ at iteration $i$ as
% \begin{equation}
% \label{eq: beta}
%     \begin{aligned}
%         \beta_i = \frac{\sum_{j\in \mathcal{Y}^{1:t}} \alpha_i^j r_i^j \nabla_{\mathcal{L}_{ce}}}{\sum_{j\in \mathcal{Y}^{1:t-1}} \nabla_{\mathcal{L}_{DAKD}}}
%     \end{aligned}
% \end{equation}
\begin{equation}
\label{eq: beta}
    \begin{aligned}
        \beta_i = \frac{||\alpha_i r_i \nabla_{\mathcal{L}_{ce}}||}{||\nabla_{\mathcal{L}_{DAKD}}||}
    \end{aligned}
\end{equation}

Therefore, the overall DGR can be formulated as in  Equation~\ref{eq: gradient-inter-phase}
\begin{equation}
\label{eq: gradient-inter-phase}
    \begin{aligned}
        W_{i+1}^{j} = W_i^{j} - \eta ( \mathrlap{\underbrace{\phantom{(\alpha^{j}_i \nabla_{\mathcal{L}_{ce}}}}_{j \in \mathcal{Y}^{t}}}
        \alpha^{j}_i r_i^j \mathrlap{\overbrace{\phantom{ \nabla_{\mathcal{L}_{ce}}(W_i^{j}) + \beta_{i} \nabla + \beta_{i} }}^{j \in \mathcal{Y}^{1:t-1}}}  \nabla_{\mathcal{L}_{ce}}(W_i^{j}) + \beta_{i} \nabla_{\mathcal{L}_{DAKD}}(W_i^{j}))
    \end{aligned}
\end{equation}

Note that in this work, we intentionally avoid re-weighting the gradients class-wise from knowledge distillation loss as it contains instrumental information obtained from previous training distribution to help maintain the discrimination of learned classes during CIL as studied in~\cite{mainatining}. In Section~\ref{subsec: ablation}, we show that re-weighting the gradients of knowledge distillation could even harm the overall performance. 
% The entire procedure for gradient reweighting is illustrated in Algorithm~\ref{alg:gr}. 




% the knowledge distillation loss $\mathcal{L}_{kd}$ encourages the model to the optimal solution from the training distribution in the last learning phase while the cross-entropy loss$\mathcal{L}makes}$ make the model adapt to new training distribution containing the old classes exemplars and new classes data. Therefore, we regard the cross-entropy as the plasticity and knowledge distillation as stability and try to balance the to strike the balance of stability and plasticity. 


% \begin{equation}
% \label{eq: gradient-inter-phase}
%     \begin{aligned}
%         W_{i+1}^{j} = W_i^{j} - \eta (\alpha^{j}_i \nabla_{\mathcal{L}_{ce}}(W_i^{j}) + \beta_{i} \nabla_{\mathcal{L}_{kd}}(W_i^{j}))
%     \end{aligned}






% the same training objective while .






% Specifically, we consider the knowledge distillation loss $\mathcal{L}_{kd}$ to maintaining the original training distribution 



% by applying the knowledge distillation loss~\cite{KD} to maintain the original training distribution, and using the phase-accumulated gradients as prior knowledge learned in earlier phases to balance the optimization process with the goal of striking the balance of stability and plasticity. 

% \subsubsection{Imbalanced Forgetting}
% \label{subsubsec: im-forgetting}
% The most intuitive way to address this is to have a  weighted sample exemplar selection. 

% \begin{equation}
% \label{eq: kd_ours}
%     \begin{aligned}
%         \mathcal{L}_{kd} = \sum_{j=1}^{|\mathcal{Y}^{1:t-1}|}\hat{p}_j log(p_j)
%     \end{aligned}
% \end{equation}




==> sec/related_work_old.tex <==
\section{Related Work}
\label{sec:related_work}
In this section, we review existing studies that are most related to our work including class-incremental learning and long-tailed imbalanced learning. 
\subsection{Class-Incremental Learning}
\label{subsec: relatedwork_cil}
Class-incremental learning (CIL) is a subarea of continual learning where the task index is not provided during the inference phase, \textit{i.e. }a single head classifier~\cite{SIT} is used for all classes seen so far. Existing CIL has been studied in both online and offline scenarios where each data is observed only once by the model in the former case. 

\textbf{Conventional CIL} approaches can be mainly categorized into three groups including regularization, memory replay, and parameter isolation. 
The \textit{regularization-based} methods aim to restrict drastic alterations to model parameters that are important for learned classes. A representative technique is to apply knowledge distillation~\cite{KD} by comparing the output logits~\cite{LWF, ICARL, EEIL, BiC} or the intermediate layers~\cite{rebalancing, douillard2020podnet, simon2021learning_featkd} between the frozen teacher model obtained from last incremental phase and the student model in the current phase, thus improving the stability during CIL. In addition, recent studies~\cite{BiC, SSIL, dualmemory} reveal the uneven norm of weight vectors learned in FC layer, which causes biased predictions towards newer learned classes. Most existing methods address this issue by applying post-hoc biased logits correction~\cite{BiC, mainatining, dualmemory, He_2022_WACV} or using separated softmax~\cite{SSIL} and cosine normalized classifier~\cite{rebalancing}.
The \textit{replay-based} methods store a small set of data from learned classes as exemplars after each incremental step to perform knowledge replay in subsequent phases instead of solely relying on new training data. Herding exemplar selection~\cite{HERDING} is widely employed in CIL~\cite{ICARL, EEIL, BiC} to select representative data based on the class mean. Later, a learning-based exemplar selection method is introduced in~\cite{liu2020mnemonics} to maximize the performance of learned knowledge further. In the online setting, the exemplar selection is performed at the end of each training iteration~\cite{GEM, A-GEM, ILIO, prabhu2020gdumb_online, NEURIPS2019_e562cd9c_GSS, NEURIPS2019_15825aee_MIR, he2022_expfree, guo2023dealing} without knowing the distribution of training data. 
Finally, the \textit{parameter isolation} related approaches gradually expand the network size or increase model parameters~\cite{DER, foster, liu2021adaptive, DEN, zenke2017continual_splitcifar} to provide dedicated space for learning new knowledge while ensuring the previously learned information remains relatively undisturbed. 

\textbf{Imbalanced CIL} remains less explored compared to conventional CIL due to the intricate challenge of addressing both catastrophic forgetting and imbalanced learning simultaneously. The earlier works focus on imbalanced continual learning under multi-label~\cite{kim2020imbalanced_PRS} and semi-supervised classification~\cite{belouadah2020active}. A class-balanced reservoir sampling (CBRS) is proposed in~\cite{chrysakis2020online} to store evenly distributed iid samples from an imbalanced datastream under online CIL. The most recent study~\cite{liu2022long} formulated long-tailed CIL for both shuffled and ordered cases and proposed a two-stage technique to decouple representation learning and classifier learning. Later, an end-to-end framework is introduced in~\cite{he2023long} by integrating exemplar augmentation with knowledge distillation. In this work, we primarily focus on long-tailed CIL~\cite{liu2022long} to address the imbalance issue from the perspective of bias correction. Instead of applying post-hoc logits adjustment~\cite{BiC, mainatining, He_2022_WACV}, we aim to directly balance the training process by reweighting the gradient updates. In addition, contrasting the findings in~\cite{kim2020imbalanced_PRS}, we observed imbalanced forgetting where the head classes instead suffer more performance degradation attributed to the larger volume of lost training data in subsequent incremental phases. Therefore, we incorporate a distribution-aware knowledge distillation loss to impose a more stringent regularization on head classes to further mitigate the forgetting issue. 

\subsection{Long-tailed Learning}
\label{subsec: relatedwork_lt}
The deep long-tailed learning for visual recognition has been studied comprehensively~\cite{zhang2021deep, yang2022survey} over the decades due to the prevalence of class-imbalanced data obtained in real-world scenarios. The major challenge arises from the fact that the performance of deep learning models tends to be dominated by head classes, leaving the learning for tail classes significantly under-realized. Existing methods can be grouped into three categories including class re-balancing, data augmentation, and module improvements. In this work, we center on class re-balanced based approaches with the goal of re-balancing the negative influence resulting from imbalanced training samples, which mainly consists of re-sampling, and class-sensitive learning. Specifically, the \textit{re-sampling} based methods~\cite{ROS, RUS_ROS, CMO} aim to construct a balanced training batch by increasing the probability of tail classes to be sampled such as random over-sampling. However, the naive sampling by simply repeating the data points may further intensify the over-fitting issues. The \textit{class-sensitive} learning seeks to adjust the value of training loss or output logits for different classes to re-balance the uneven learning effects by re-weighting class influence based on label frequencies~\cite{cui2019class, BSLoss, LDAM, IBLoss, logit_adjust}. In addition, recent studies~\cite{tan2020equalizationv1, tan2021equalizationv2, guo2023dealing} argue that the imbalance of positive and negative gradients severely inhibits balanced learning and they seek to up-weight the positive gradients and down-weight the negative gradients for different classes. Our proposed method stems from a similar observation where the magnitude of gradient vectors diverges significantly between head and tail classes during the learning process. This discrepancy leads to uneven optimization steps, subsequently causing the model to overfit the head classes while underfitting the tail classes. To address this, our goal is to equilibrate the gradient updates, ensuring a more balanced learning process. Furthermore, existing long-tailed learning methods do not consider previously acquired knowledge in learned classes, making them unsuitable under the context of CIL. 
